Epistemic Logic with Functional Dependency Operator

Epistemic logic with non-standard knowledge operators, especially the "knowing-value" operator, has recently gathered much attention. With the "knowing-value" operator, we can express knowledge of individual variables, but not of the relations between them in general. In this paper, we propose a new operator Kf to express knowledge of the functional dependencies between variables. The semantics of this Kf operator uses a function domain which imposes a constraint on what counts as a functional dependency relation. By adjusting this function domain, different interesting logics arise, and in this paper we axiomatize three such logics in a single agent setting. Then we show how these three logics can be unified by allowing the function domain to vary relative to different agents and possible worlds. A multiagent axiomatization is given in this case.

==> UsualMacros.tex <==
%%% Universal Macros
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\rel}[1]{\stackrel{#1}{\rightarrow}}
\newcommand{\lr}[1]{\langle #1 \rangle}
\newcommand{\llrr}[1]{\{ #1 \}}
\newcommand{\sep}{\ |\ }
\newcommand{\Mod}{\mathrm{Mod}}
\newcommand{\Ind}{\mathrm{Ind}}
\newcommand{\oln}{\overline}
\newcommand{\join}{\bigvee}
\newcommand{\meet}{\bigwedge}
\newcommand{\Dia}{\Diamond}
\newcommand{\lra}{\leftrightarrow}
\newcommand{\uar}{\vec}
\newcommand{\straightphi}{\phi}
\renewcommand{\phi}{\varphi}
\newcommand{\todo}[1]{\textcolor{red}{\textbf{[ TODO: #1 ]}}}
